Sparse Coral Classification Using Deep Convolutional Neural Networks

Autonomous repair of deep-sea coral reefs is a recent proposed idea to support the oceans ecosystem in which is vital for commercial fishing, tourism and other species. This idea can be operated through using many small autonomous underwater vehicles (AUVs) and swarm intelligence techniques to locate and replace chunks of coral which have been broken off, thus enabling re-growth and maintaining the habitat. The aim of this project is developing machine vision algorithms to enable an underwater robot to locate a coral reef and a chunk of coral on the seabed and prompt the robot to pick it up. Although there is no literature on this particular problem, related work on fish counting may give some insight into the problem. The technical challenges are principally due to the potential lack of clarity of the water and platform stabilization as well as spurious artifacts (rocks, fish, and crabs). We present an efficient sparse classification for coral species using supervised deep learning method called Convolutional Neural Networks (CNNs). We compute Weber Local Descriptor (WLD), Phase Congruency (PC), and Zero Component Analysis (ZCA) Whitening to extract shape and texture feature descriptors, which are employed to be supplementary channels (feature-based maps) besides basic spatial color channels (spatial-based maps) of coral input image, we also experiment state-of-art preprocessing underwater algorithms for image enhancement and color normalization and color conversion adjustment. Our proposed coral classification method is developed under MATLAB platform, and evaluated by two different coral datasets (University of California San Diego's Moorea Labeled Corals, and Heriot-Watt University's Atlantic Deep Sea).

==> Ch2_Literature_Review.tex <==
\chapter{Problem Definition} \label{chap:problem}

Marcos [15] developed an automated rapid classification (5 classes: coral, sand, rubble, dead coral, and dead coral with algae) for underwater reef video, he used color features based on histogram of normalized chromaticity coordinates (NCC) and texture features from local binary patterns (LBP) descriptor, those features feed into linear discriminant analysis (LDA) classifier, in case of using more classes [16]; his method outputs inaccurate classification . Pizarro [17] introduced object recognition for coarse habitat classification (1st experiment; 8 classes: coralline rubble, hard coral, hard coral +soft coral + coralline rubble, halimeda + hard Coral + coralline rubble, macroalgae, rhodolith, sponges, and un-colonized) (2nd experiment; 4 classes: reef + coarse sand, coarse sand, reef, and fine sand), he employed the same color features of Marcos but different texture features based on bag-of-words using scale-invariant feature transform (SIFT) with extra saliency feature of gabor-filter response, this method can be only used with single-object images (one classes per entire image) [16].
Strokes [18] describes an automated computer algorithm for the classification of coral reef benthic organisms and substrates which divides image into blocks, then find distance between those blocks and identified species blocks based on color features (normalized histogram of RGB color space) and texture features (radial samples of 2D discrete cosine transform) by using inconvenient distance metric (manually assigned parameters) after unsuccessful results of well-known mahalanobis distance. Beijbom [19] introduced Moorea Labeled Corals (MLC) dataset and proposed multi-scale classification algorithm for automatic annotation, he developed color stretching for each channel individually in L*a*b* color space as pre-processing step, then uses Maximum Response (MR) filter bank approach (rotation invariant) as color and texture feature, followed by applying Radial Basis Function kernel (RBF) of Support Vector Machines (SVM) classifier, this method seeks all possibilities (time-consuming) to find a suitable patch size around selected image points for species identification.
Shihavuddin [16] implemented hybrid variable-scheme classification framework for benthic coral reef images or mosaics, this framework uses combination of the following features (local binary pattern (CLBP), grey level co-occurrence matrix (GLCM), Gabor filter response, and opponent angle and hue channel color histograms) and also combination of the following classifiers (k- nearest neighbor (KNN), neural network (NN), support vector machine (SVM) or probability density weighted mean distance (PDWMD)) along besides middleware procedures for better result enhancement, but this framework works sufficiently with small-patched images (high negative impact of background information).
Stough [20] presented an automatic binary segmentation technique of live Staghorn coral species, in which regional intensity quantile functions (QF) is used as color features and Scale-Invariant Feature Transform (SIFT) is maintained to be texture features, followed by linear SVM as classifier, this supervised technique is highly noise sensitive (due to SIFT). Purser [21] investigated machine-learning algorithms for the automated detection of cold-water coral habitats, which computes 15 differently oriented and spaced gratings in order to produce a set of 30 texture features, and to compare a computer vision system with the use of three manual methods: 15-point quadrat, 100-point quadrat and frame mapping. Johnson-Roberson [22] shows an approach for the autonomous segmentation and classification of coral through the combination of visual and acoustic data, which generates 60 visual features: 12 are the mean and standard deviation of all of the RGB and HSV channels separately and the remaining 48 are obtained by convolving the region with Gabor wavelets at six scales and four orientations and taking the mean and standard deviation of the results for each scale and orientation combination, then SVM is selected for classification task, pre-processing is mainly required to allocate foreground regions before feature extraction.
Schoening et al. [23] introduced semi-automated detection system for deep-sea coral images, in which firstly applies preprocessing step for illumination correction, then secondly extracts high dimensional features at labeled pixels based on MPEG7 standard (four descriptors for color features; three for texture; ten for structure and motion), after that a set of successive different support vector machines is applied a long side with thresholding post processing, although the used features are more generic for any application leading to high sensitivity for underwater cluttering background. 
Clement [24] presented local binary pattern (LBP) as feature descriptor for binary detection of crown-of-thorns starfish (COTS) from great barrier reef images in Australia, in which his experiments achieved an above-average results in only one-class segmentation.
 Mehta [25] used support vector machines (SVM) classifier directly on spatial information of coral image without any preprocessing step to get a binary (coral/non-coral) output, he reasoned for using raw-data as classifier input such that features and descriptors for coral textures are very difficult to obtain. he achieved 95 \%  correct classification but his method behaves negatively with any change in underwater illumination.

Rather than depending on human-crafted features to get a proper coral classification, the proposed work decides letting the feature mapping to be done automatically by deep convolutional neural networks regardless to any under-water environment condition. by feeding new images, the network can learn and adapt the constructed feature maps respect to desired class outputs.

==> Ch3_CNN.tex <==
\chapter{State of the art} \label{chap:state}

\section{Introduction} 

\section{Recent Work}

\section{Applications}

\section{Summary}

==> Ch4_Proposed_Framework.tex <==
\chapter{Methodology} \label{chap:method}

\section{Introduction}

Coral-reef classification can be divided into three main consecutive steps:
\begin{enumerate}
\item Under-water image de-noising (preprocessing step): Due to different challenges (motion blurring, color attenuation, refracted sunlight patterns, water temperature variation, sky color variation, scattering effects, presence of sea particles, etc... ),  raw image must be enhanced visually to show its coral species in details for further steps.
\item Feature extraction: image which contains different coral species, have to find salient regions in each object in order to identify and distinguish those species easily respect to invariance of the following aspects (illumination, rotation, size, view angle, camera distance, etc ...).
\item Machine Learning (ML) algorithm: those extracted features are used as input for machine learning to find suitable parameters to converge species of new images to similar trained ones respectively.
\end{enumerate}

Proposed work consists of two stages: offline data training and online identification. offline training will be on surface workstation for fast computation and long execution time which extracts features from coral-labeled images using Phase Congruency and then apply deep learning process (supervised, unsupervised, or hybrid) to get well-trained parameter for further successful classification. However, online identification will be on remotely operated underwater vehicle (ROV) which collect images from several coralbots and find out which species are included and detect their coordinates in real-time processing. 

\section{Framework Overview}

\section{Implementation}

\subsection{Preprocessing}
\subsection{Feature Maps}
\subsubsection{Phase Congruency}
Phase Congruency \cite{Morrone1988,Oppenheim1981} represent image features in such format which should be high in information and low in redundancy using Fourier transform, rather than set of edges (sharp changes in intensity). in other words, Phase Congruency \cite{Zhang2012} is a dimensionless measure for the of a image structure independently of the signal amplitude which is based on Kovesi’s work \cite{Kovesi1999}. Those features are fully invariant to image illumination and contrast, and also partially invariant  to scale and rotation transformation in case of application of suitable normalization process in frequency domain \cite{Burlacu2008}.
\subsection{Network Architecture}

\section{Summary}

==> background.tex <==
\chapter{Background} \label{chap:background}

\section{Introduction}
Many scientific subject areas (i.e. medicine, remote sensing) have
to deal with the problem of image correspondence (also known as
image registration or image matching). This problem arises when
there is a need to extract information about an object by
comparing a set of different images in which this object appears.
Most of the time this comparison cannot be performed easily
because of differences between images such as viewpoint changes,
use of different sensors, images taken at different times, and
changes in general imaging conditions. Given such differences, a
way to align different images of the same object is needed. In
medical applications, and specifically in mammography,
radiologists have to deal with all the above problems. For
example, a way to detect abnormal structures in the breast is to
compare temporal (images of the same breast taken at different
times) or contralateral (using left-right breast) mammograms.

As images are taken under different conditions (i.e. film
sensitivity, radiation exposure, breast compression and patient
movement) and/or time intervals (e.g. screening interval of three
years) the structure of the breast is likely to suffer some
changes, although an overall similarity will be maintained. A way
to detect those changes is to align the images and compare the
results using, for instance, simple image subtraction. In
addition, as described in the previous chapter, different imaging
modalities are being used to provide a better understanding of a
region of interest. The first step to incorporate information from
those modalities is to align them to be able to establish areas of
correspondence.

An image correspondence method is based on finding a mapping
function ($f(x,y)$) that maps each coordinate of one image ($A$)
into another image ($B$).

\begin{equation}
B(x',y')=A(f(x,y))
\end{equation}
\noindent which maps spatial coordinates $(x,y)$ in the reference
image $A$ to coordinates $(x',y')$ in the warped (also referred to
as target) image $B$. Usually the function $f$ is expressed as two
(or three in three dimensions) separate functions $f_x$ and $f_y$
(and $f_z$). This review describes image registration in two
dimensions. However extrapolation to 3D is often straightforward
and is described in detail where appropriate.

A general methodology for image alignment typically follows those
steps:

\begin{enumerate}
\item \emph{Selection and extraction of features.} A registration method can
be based on matching different image primitives. For instance
points, edges, ridges, surfaces, or a whole image. The selection
of a suitable primitive is a trade off between the information it
provides and its complexity. For instance, raw pixels with only
intensity information provide a straightforward comparison. On the
other hand, taking the whole image provides more (and more
complex) information. Primitives will be described by a set of
features extracted from them. That is the case, for instance, of
shape features extracted from regions or curvature values
extracted from linear structures. There is an extensive literature
about feature extraction, the reader is referred to Chapter 4
where a review on that subject is given.

\item \emph{Similarity metric.} A way to measure the similarity between
the extracted features is needed. Many different similarity
metrics have been proposed and their suitability depends on the
chosen feature. The reader is referred to Chapter 5 where
similarity measures are reviewed and a novel measure is proposed.

\item \emph{Selection of the mapping function and estimation of
its parameters.} The complexity of a mapping function should be
determined depending on the application field and type of
misalignment we are dealing with. Once a mapping function is
selected its parameters need to be estimated. This requires a
definition of an optimum search space and search strategy which is
often related to optimisation of a cost function related to a
similarity measure previously mentioned.

\item \emph{Alignment of images using the mapping function.} When the
function parameters are known we are able to transform an image in
order to minimise the initial misalignment.
\end{enumerate}


\subsection{Interpolation}
Usually transformed coordinates $(x',y')$ in the warped image do
not match a given coordinate grid (i.e. they are non-integer
values) and interpolation is needed. Different interpolation
methods have been used in image registration: nearest neighbour,
tri-linear and partial volume distribution. The interpolation
problem is graphically represented in Figure~\ref{fig:interp}.

\begin{figure}[htb]
        \centering
        \epsfxsize=4cm
        {\epsfbox{figures/interp.eps}}
  \caption{Interpolation of corresponding coordinates}
  \label{fig:interp}
\end{figure}

Nearest neighbour interpolation assigns the intensity value of
$m=(x',y')$ to its nearest point:
\begin{equation}
        B(m)=B(\_{\forall i}{min}(d_E[m,n_i]))
\end{equation}
\noindent where $d_E$ indicates Euclidean distance and $n_i$ are
the nearest neighbours. The nearest neighbour approach provides
good accuracy and it is easy to compute.

Trilinear interpolation assigns to $m$ the value of the weighted
($w_i$) sum of the neighbouring pixels.

\begin{equation}
        B(m)=\sum_iw_i B(n_i)
\end{equation}
\noindent where each weight $w_i$ is related to the distance from
$m$ (see Figure~\ref{fig:interp})

\begin{equation}
        w_1 = (1-dx)(1-dy) ~~~~ w_2 = (1-dx)dy ~~~~w_3 = dx(1-dy)
        ~~~~ w_4 = dx dy
        \nonumber
\end{equation}

This interpolation creates a new intensity value, which could
introduce undesirable effects in the intensity distribution. This
fact is regarded as its main drawback, and can be solved using a
partial volume distribution. This method adds the weight of each
neighbour ($w_i$ values) at the intensity value in the histogram
distribution, without creating an additional intensity value.


==> intro.tex <==
\chapter{Introduction} \label{chap:intro}

\section{Background} \label{sect:bkgrnd}

\section{Problem Definition}

\section{Challenges}

\section{Thesis Outline}

